Parameterized Model-Checking for Timed-Systems with Conjunctive Guards (Extended Version)

In this work we extend the Emerson and Kahlon's cutoff theorems for process skeletons with conjunctive guards to Parameterized Networks of Timed Automata, i.e. systems obtained by an \emph{apriori} unknown number of Timed Automata instantiated from a finite set $U_1, \dots, U_n$ of Timed Automata templates. In this way we aim at giving a tool to universally verify software systems where an unknown number of software components (i.e. processes) interact with continuous time temporal constraints. It is often the case, indeed, that distributed algorithms show an heterogeneous nature, combining dynamic aspects with real-time aspects. In the paper we will also show how to model check a protocol that uses special variables storing identifiers of the participating processes (i.e. PIDs) in Timed Automata with conjunctive guards. This is non-trivial, since solutions to the parameterized verification problem often relies on the processes to be symmetric, i.e. indistinguishable. On the other side, many popular distributed algorithms make use of PIDs and thus cannot directly apply those solutions.

==> figures/Makefile <==
DIA=`which dia`
MPOST=`which mpost`

all : mps eps fig
#all : png mps eps fig

fig : fig1 fig2 fig3 fig4 fig5 fig6 fig7 fig8 fig9 fig10 \
	fig11 fig12 fig13 fig14 fig15 fig16 fig17 fig18 fig19

eps : owner.eps owner_safe.eps condor_chirp.eps starter.eps \
	submit.eps shadow.eps chirp_read.eps intruder.eps \
	schedd.eps schedd_sock-A-trust.eps schedd_sock-A-nottrust.eps \
	A-LTS.eps H-LTS.eps I-LTS.eps simple_system.eps product_system.eps


png : owner.png owner_safe.png condor_chirp.png starter.png \
	submit.png shadow.png chirp_read.png intruder.png \
	schedd.png schedd_sock-A-trust.png schedd_sock-A-nottrust.png \
	A-LTS.png H-LTS.png I-LTS.png simple_system.png product_system.png


mps : owner.mps owner_safe.mps condor_chirp.mps starter.mps \
	submit.mps shadow.mps chirp_read.mps intruder.mps \
	schedd.mps schedd_sock-A-trust.mps schedd_sock-A-nottrust.mps \
	A-LTS.mps H-LTS.mps I-LTS.mps simple_system.mps product_system.mps

#simple_system
simple_system.mps : simple_system.dia
	rm -f simple_system.1 simple_system.mp
	${DIA} -e simple_system.mp simple_system.dia
	${MPOST} simple_system.mp
	mv simple_system.1 simple_system.mps
	rm simple_system.mpx simple_system.log simple_system.mp
	
simple_system.png : simple_system.eps
	convert simple_system.eps simple_system.png

#product_system
product_system.mps : product_system.dia
	rm -f product_system.1 product_system.mp
	${DIA} -e product_system.mp product_system.dia
	${MPOST} product_system.mp
	mv product_system.1 product_system.mps
	rm product_system.mpx product_system.log product_system.mp
	
product_system.png : product_system.eps
	convert product_system.eps product_system.png




#I-LTS
I-LTS.mps : I-LTS.dia
	rm -f I-LTS.1 I-LTS.mp
	${DIA} -e I-LTS.mp I-LTS.dia
	${MPOST} I-LTS.mp
	mv I-LTS.1 I-LTS.mps
	rm I-LTS.mpx I-LTS.log I-LTS.mp
	
I-LTS.png : I-LTS.eps
	convert I-LTS.eps I-LTS.png


#A-LTS
A-LTS.mps : A-LTS.dia
	rm -f A-LTS.1 A-LTS.mp
	${DIA} -e A-LTS.mp A-LTS.dia
	${MPOST} A-LTS.mp
	mv A-LTS.1 A-LTS.mps
	rm A-LTS.mpx A-LTS.log A-LTS.mp
	
A-LTS.png : A-LTS.eps
	convert A-LTS.eps A-LTS.png

#H-LTS
H-LTS.mps : H-LTS.dia
	rm -f H-LTS.1 H-LTS.mp
	${DIA} -e H-LTS.mp H-LTS.dia
	${MPOST} H-LTS.mp
	mv H-LTS.1 H-LTS.mps
	rm H-LTS.mpx H-LTS.log H-LTS.mp
	
H-LTS.png : H-LTS.eps
	convert H-LTS.eps H-LTS.png


#intruder
intruder.mps : intruder.dia
	rm -f intruder.1 intruder.mp
	${DIA} -e intruder.mp intruder.dia
	${MPOST} intruder.mp
	mv intruder.1 intruder.mps
	rm intruder.mpx intruder.log intruder.mp
	
intruder.png : intruder.eps
	convert intruder.eps intruder.png

intruder.pdf : intruder.eps
	epstopdf intruder.eps

#
#owner
owner.mps : owner.dia
	rm -f owner.1 owner.mp
	${DIA} -e owner.mp owner.dia
	${MPOST} owner.mp
	mv owner.1 owner.mps
	rm owner.mpx owner.log owner.mp
	
owner.png : owner.eps
	convert owner.eps owner.png

owner.pdf : owner.eps
	epstopdf owner.eps

#
#owner_safe
owner_safe.mps : owner_safe.dia
	rm -f owner_safe.1 owner_safe.mp
	${DIA} -e owner_safe.mp owner_safe.dia
	${MPOST} owner_safe.mp
	mv owner_safe.1 owner_safe.mps
	rm owner_safe.mpx owner_safe.log owner_safe.mp
	
owner_safe.png : owner_safe.eps
	convert owner_safe.eps owner_safe.png

#chirp_read
chirp_read.mps : chirp_read.dia
	rm -f chirp_read.1 chirp_read.mp
	${DIA} -e chirp_read.mp chirp_read.dia
	${MPOST} chirp_read.mp
	mv chirp_read.1 chirp_read.mps
	rm chirp_read.mpx chirp_read.log chirp_read.mp
	
chirp_read.png : chirp_read.eps
	convert chirp_read.eps chirp_read.png

chirp_read.pdf : chirp_read.eps
	epstopdf chirp_read.eps

#condor_chirp
condor_chirp.mps : condor_chirp.dia
	rm -f condor_chirp_set_onwer.mp condor_chirp.1
	${DIA} -e condor_chirp.mp condor_chirp.dia
	${MPOST} condor_chirp.mp
	mv condor_chirp.1 condor_chirp.mps
	rm condor_chirp.mpx condor_chirp.log condor_chirp.mp

condor_chirp.png : condor_chirp.eps
	convert condor_chirp.eps condor_chirp.png

condor_chirp.pdf : condor_chirp.eps
	epstopdf condor_chirp.eps 

#starter
starter.mps : starter.dia
	rm -f starter.mp starter.1
	${DIA} -e starter.mp starter.dia
	${MPOST} starter.mp
	mv starter.1 starter.mps
	rm starter.mpx starter.log starter.mp

starter.pdf : starter.eps
	epstopdf starter.eps

starter.png : starter.eps
	convert starter.eps starter.png

#submit
submit.mps : submit.dia
	rm -f submit.mp submit.1
	${DIA} -e submit.mp submit.dia
	${MPOST} submit.mp
	mv submit.1 submit.mps
	rm submit.mpx submit.log submit.mp

submit.png : submit.eps
	convert submit.eps submit.png

submit.pdf : submit.eps
	epstopdf submit.eps

#shadow
shadow.mps : shadow.dia
	rm -f shadow.mp shadow.1
	${DIA} -e shadow.mp shadow.dia
	${MPOST} shadow.mp
	mv shadow.1 shadow.mps
	rm shadow.mpx shadow.log shadow.mp

shadow.png : shadow.eps
	convert shadow.eps shadow.png

shadow.pdf : shadow.eps
	epstopdf shadow.eps

#schedd
schedd.mps : schedd.dia
	rm -f schedd.mp schedd.1
	${DIA} -e schedd.mp schedd.dia
	${MPOST} schedd.mp
	mv schedd.1 schedd.mps
	rm schedd.mpx schedd.log schedd.mp

schedd.png : schedd.eps
	convert schedd.eps schedd.png

schedd.pdf : schedd.eps
	epstopdf schedd.eps

#schedd_sock-A-trust
schedd_sock-A-trust.mps : schedd_sock-A-trust.dia
	rm -f schedd_sock-A-trust.mp schedd_sock-A-trust.1
	${DIA} -e schedd_sock-A-trust.mp schedd_sock-A-trust.dia
	${MPOST} schedd_sock-A-trust.mp
	mv schedd_sock-A-trust.1 schedd_sock-A-trust.mps
	rm schedd_sock-A-trust.mpx schedd_sock-A-trust.log schedd_sock-A-trust.mp

schedd_sock-A-trust.png : schedd_sock-A-trust.eps
	convert schedd_sock-A-trust.eps schedd_sock-A-trust.png

schedd_sock-A-trust.pdf : schedd_sock-A-trust.eps
	epstopdf schedd_sock-A-trust.eps

#schedd_sock-A-nottrust
schedd_sock-A-nottrust.mps : schedd_sock-A-nottrust.dia
	rm -f schedd_sock-A-nottrust.mp schedd_sock-A-nottrust.1
	${DIA} -e schedd_sock-A-nottrust.mp schedd_sock-A-nottrust.dia
	${MPOST} schedd_sock-A-nottrust.mp
	mv schedd_sock-A-nottrust.1 schedd_sock-A-nottrust.mps
	rm schedd_sock-A-nottrust.mpx schedd_sock-A-nottrust.log schedd_sock-A-nottrust.mp

schedd_sock-A-nottrust.png : schedd_sock-A-nottrust.eps
	convert schedd_sock-A-nottrust.eps schedd_sock-A-nottrust.png

schedd_sock-A-nottrust.pdf : schedd_sock-A-nottrust.eps
	epstopdf schedd_sock-A-nottrust.eps

# clean all
clean :
	rm -f *.1 *.mp *.mps *.log *.mpx *.png mpxerr.te *.eps *.tex *.ps *.dvi *.aux fig*.eps

# ====
# create eps
# ====

submit.eps : submit.mps metapost2eps.tex.template
	cat metapost2eps.tex.template | sed -e 's/<imagefile>/submit/' > submit.tex
	latex submit.tex
	dvips submit.dvi
	ps2eps -f submit.ps
	rm -f submit.tex submit.dvi submit.ps
	cp submit.eps ../figures/fig9.eps


owner.eps : owner.mps metapost2eps.tex.template
	cat metapost2eps.tex.template | sed -e 's/<imagefile>/owner/' > owner.tex
	latex owner.tex
	dvips owner.dvi
	ps2eps -f owner.ps
	rm -f owner.tex owner.dvi owner.ps

owner_safe.eps : owner_safe.mps metapost2eps.tex.template
	cat metapost2eps.tex.template | sed -e 's/<imagefile>/owner_safe/' > owner_safe.tex
	latex owner_safe.tex
	dvips owner_safe.dvi
	ps2eps -f owner_safe.ps
	rm -f owner_safe.tex owner_safe.dvi owner_safe.ps

condor_chirp.eps : condor_chirp.mps metapost2eps.tex.template
	cat metapost2eps.tex.template | sed -e 's/<imagefile>/condor_chirp/' > condor_chirp.tex
	latex condor_chirp.tex
	dvips condor_chirp.dvi
	ps2eps -f condor_chirp.ps
	rm -f condor_chirp.tex condor_chirp.dvi condor_chirp.ps

starter.eps : starter.mps metapost2eps.tex.template
	cat metapost2eps.tex.template | sed -e 's/<imagefile>/starter/' > starter.tex
	latex starter.tex
	dvips starter.dvi
	ps2eps -f starter.ps
	rm -f starter.tex starter.dvi starter.ps


shadow.eps : shadow.mps metapost2eps.tex.template
	cat metapost2eps.tex.template | sed -e 's/<imagefile>/shadow/' > shadow.tex
	latex shadow.tex
	dvips shadow.dvi
	ps2eps -f shadow.ps
	rm -f shadow.tex shadow.dvi shadow.ps

chirp_read.eps : chirp_read.mps metapost2eps.tex.template
	cat metapost2eps.tex.template | sed -e 's/<imagefile>/chirp_read/' > chirp_read.tex
	latex chirp_read.tex
	dvips chirp_read.dvi
	ps2eps -f chirp_read.ps
	rm -f chirp_read.tex chirp_read.dvi chirp_read.ps
	cp chirp_read.eps ../figures/fig5.eps

intruder.eps : intruder.mps metapost2eps.tex.template
	cat metapost2eps.tex.template | sed -e 's/<imagefile>/intruder/' > intruder.tex
	latex intruder.tex
	dvips intruder.dvi
	ps2eps -f intruder.ps
	rm -f intruder.tex intruder.dvi intruder.ps

schedd.eps : schedd.mps metapost2eps.tex.template
	cat metapost2eps.tex.template | sed -e 's/<imagefile>/schedd/' > schedd.tex
	latex schedd.tex
	dvips schedd.dvi
	ps2eps -f schedd.ps
	rm -f schedd.tex schedd.dvi schedd.ps

schedd_sock-A-trust.eps : schedd_sock-A-trust.mps metapost2eps.tex.template
	cat metapost2eps.tex.template | sed -e 's/<imagefile>/schedd_sock-A-trust/' > schedd_sock-A-trust.tex
	latex schedd_sock-A-trust.tex
	dvips schedd_sock-A-trust.dvi
	ps2eps -f schedd_sock-A-trust.ps
	rm -f schedd_sock-A-trust.tex schedd_sock-A-trust.dvi schedd_sock-A-trust.ps

schedd_sock-A-nottrust.eps : schedd_sock-A-nottrust.mps metapost2eps.tex.template
	cat metapost2eps.tex.template | sed -e 's/<imagefile>/schedd_sock-A-nottrust/' > schedd_sock-A-nottrust.tex
	latex schedd_sock-A-nottrust.tex
	dvips schedd_sock-A-nottrust.dvi
	ps2eps -f schedd_sock-A-nottrust.ps
	rm -f schedd_sock-A-nottrust.tex schedd_sock-A-nottrust.dvi schedd_sock-A-nottrust.ps

A-LTS.eps : A-LTS.mps metapost2eps.tex.template
	cat metapost2eps.tex.template | sed -e 's/<imagefile>/A-LTS/' > A-LTS.tex
	latex A-LTS.tex
	dvips A-LTS.dvi
	ps2eps -f A-LTS.ps
	rm -f A-LTS.tex A-LTS.dvi A-LTS.ps

H-LTS.eps : H-LTS.mps metapost2eps.tex.template
	cat metapost2eps.tex.template | sed -e 's/<imagefile>/H-LTS/' > H-LTS.tex
	latex H-LTS.tex
	dvips H-LTS.dvi
	ps2eps -f H-LTS.ps
	rm -f H-LTS.tex H-LTS.dvi H-LTS.ps
	cp H-LTS.eps ../figures/fig6.eps

I-LTS.eps : I-LTS.mps metapost2eps.tex.template
	cat metapost2eps.tex.template | sed -e 's/<imagefile>/I-LTS/' > I-LTS.tex
	latex I-LTS.tex
	dvips I-LTS.dvi
	ps2eps -f I-LTS.ps
	rm -f I-LTS.tex I-LTS.dvi I-LTS.ps
	cp I-LTS.eps ../figures/fig7.eps

simple_system.eps : simple_system.mps metapost2eps.tex.template
	cat metapost2eps.tex.template | sed -e 's/<imagefile>/simple_system/' > simple_system.tex
	latex simple_system.tex
	dvips simple_system.dvi
	ps2eps -f simple_system.ps
	rm -f simple_system.tex simple_system.dvi simple_system.ps

product_system.eps : product_system.mps metapost2eps.tex.template
	cat metapost2eps.tex.template | sed -e 's/<imagefile>/product_system/' > product_system.tex
	latex product_system.tex
	dvips product_system.dvi
	ps2eps -f product_system.ps
	rm -f product_system.tex product_system.dvi product_system.ps

fig1 : grid_arch.pdf
	pdf2ps grid_arch.pdf
	ps2eps -f grid_arch.ps
	cp grid_arch.eps ../figures/fig1.eps

fig2 : simple_system.eps
	cp simple_system.eps ../figures/fig2.eps

fig3 : product_system.eps
	cp product_system.eps ../figures/fig3.eps

fig4 : methodology.pdf
	pdf2ps methodology.pdf
	ps2eps -f methodology.ps
	cp methodology.eps ../figures/fig4.eps

fig5 : A-LTS.eps
	cp A-LTS.eps ../figures/fig5.eps
fig6 : H-LTS.eps
	cp H-LTS.eps ../figures/fig6.eps
fig7 : I-LTS.eps
	cp I-LTS.eps ../figures/fig7.eps
fig8 : condor-protocol.pdf
	pdf2ps condor-protocol.pdf
	ps2eps -f condor-protocol.ps
	cp condor-protocol.eps ../figures/fig8.eps
fig9 : submit.eps
	cp submit.eps ../figures/fig9.eps
fig10 : starter.eps
	cp starter.eps ../figures/fig10.eps
fig11 : shadow.eps
	cp shadow.eps ../figures/fig11.eps
fig12 : condor_chirp.eps
	cp condor_chirp.eps ../figures/fig12.eps
fig13 : schedd.eps
	cp schedd.eps ../figures/fig13.eps
fig14 : schedd_sock-A-trust.eps
	cp schedd_sock-A-trust.eps ../figures/fig14.eps
fig15 : schedd_sock-A-nottrust.eps
	cp schedd_sock-A-nottrust.eps ../figures/fig15.eps
fig16 : owner.eps
	cp owner.eps ../figures/fig16.eps
fig17 : chirp_read.eps
	cp chirp_read.eps ../figures/fig17.eps
fig18 : intruder.eps
	cp intruder.eps ../figures/fig18.eps
fig19 : owner_safe.eps
	cp owner_safe.eps ../figures/fig19.eps


